BrainTalker: Low-Resource Brain-to-Speech Synthesis with Transfer Learning using Wav2Vec 2.0

Decoding spoken speech from neural activity in the brain is a fast-emerging research topic, as it could enable communication for people who have difficulties with producing audible speech. For this task, electrocorticography (ECoG) is a common method for recording brain activity with high temporal resolution and high spatial precision. However, due to the risky surgical procedure required for obtaining ECoG recordings, relatively little of this data has been collected, and the amount is insufficient to train a neural network-based Brain-to-Speech (BTS) system. To address this problem, we propose BrainTalker-a novel BTS framework that generates intelligible spoken speech from ECoG signals under extremely low-resource scenarios. We apply a transfer learning approach utilizing a pre-trained self supervised model, Wav2Vec 2.0. Specifically, we train an encoder module to map ECoG signals to latent embeddings that match Wav2Vec 2.0 representations of the corresponding spoken speech. These embeddings are then transformed into mel-spectrograms using stacked convolutional and transformer-based layers, which are fed into a neural vocoder to synthesize speech waveform. Experimental results demonstrate our proposed framework achieves outstanding performance in terms of subjective and objective metrics, including a Pearson correlation coefficient of 0.9 between generated and ground truth mel spectrograms. We share publicly available Demos and Code.

==> 2_Related_works.tex <==
\section{Related work}
\label{sec:related_works}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2.1 Spoken speech decoding from brain activity
    % 2.1.1 Edward chang and densely connected paper
% 2.2 Transfer learning
    % 2.2.2 BTS utilizing pre-trained image classification
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Brain-to-speech (BTS) synthesis}
Recent advances in deep neural network have significantly improved the performance of brain-to-speech (BTS) systems.
Those systems commonly estimate acoustic features such as mel spectrogram from brain activities \cite{anumanchipalli2019speech, angrick2019speech}. 
% edward chang
For example, \cite{anumanchipalli2019speech} estimates mel spectrogram from the neural activities by adopting a two-stage pipeline.
First, they estimate intermediate articulatory features from neural activities, and then reconstruct the target mel spectrogram using the estimated articulatory features.
Although these approaches show the potential of reconstructing spoken speech from ECoG signal, they utilize long length of recorded data for speech synthesis. 
In~\cite{angrick2019speech}, they adopt DenseNet architecture to reconstruct mel spectrogram from the ECoG signal and then synthesize speech waveform using WaveNet vocoder from the reconstructed mel spectrogram. 
In~\cite{berezutskaya2022direct}, they reconstruct speech from sensorimotor brain activity using three deep neural networks; multi-layer perceptron, DenseNet and RNN. 
However, the aforementioned studies neglected to report any subjective assessment of the synthesized speech, i.e Mean Opinion Score (MOS), thereby precluding an evaluation of the speech's perceptual quality.

Since collecting a lengthy ECoG-speech data parallelly is an extremely challenging task in real world, it is meaningful to find a way to tackle the data deficiency problem to synthesize high quality speech.
To this end, we propose a novel BTS framework adopting transfer learning~\cite{pan2020transfer} to generate high-quality speech even with 2-minutes long recordings.

\subsection{Transfer learning for brain-related feature extraction}
To tackle the data shortage problem, there are several approaches applying transfer learning for brain feature extraction.
In \cite{sadiq2022exploiting, shalbaf2020transfer, narin2022detection}, pre-trained image classification networks are utilized to obtain latent features from EEG signal.
To convert 1-dimensional EEG signal into 2-dimensional image features, they apply continuous wavelet transform (CWT)\cite{aguiar2014continuous} and calculate its absolute value to obtain scalogram\cite{kofsky1966scalogram}.
% To convert 1-dimensional EEG signal into 2-dimensional features, continuous wavelet transform (CWT)~\cite{aguiar2014continuous} is applied and calcuate the absolute value to obtain scalogram~\cite{kofsky1966scalogram}. 
Next, the scalogram is resized to match the input size of pre-trained image classification networks.
Continually, a downstream task is performed according to the purpose of each task. 

% jkyung: 위에 언급한 classification모델들이 phase 정보를 없앴다라는 점을 어필하기보다, 단순한 classification model과 비교했을 때 self-supervised로 train된 모델의 장점을 어필하는 것이 좋아보임 (아래 예시 첨부)
Although the pre-trained image classification network can be a good option for extracting the representations from neural activities, they are typically trained on labeled data for a specific task (e.g., such as object recognition or classification),
so the models may not be as effective to extract generalized features when the data distribution differs significantly from the training data.
Instead, self-supervised models, which are trained on large amounts of unlabeled data, allowing them to learn abundant representations of the input data. 
Also, scalogram feature has severe information loss such as phase, which is essential for decoding speech signal, owing to the process that takes the absolute value of CWT transformed signal.
To this end, we adopt the prominent self-supervised pre-trained model, Wav2Vec 2.0 as feature extractor, which is trained using a large amount of speech data in a self-supervised manner to capture relevant features, enabling amply utilizing the magnitude and phase information of the 1-dimensional brain signals. 

\begin{comment}
Although the pre-trained image classification network works reasonably well for extracting the representations from neural activities. However, this process also loses important information for decoding speech signal, phase, due to taking the absolute value to CWT transformed signal.
To fully utilize the magnitude and phase information of brain signals, we adopt the pre-trained model, Wav2vec2.0, which is one of the useful representation networks in speech applications. 
jkyung: 아래 문장이 논리적으로 약간의 오류가 있다고 판단됨
Since Wav2vec fully utilizes 1-dimensional time-domain signal as an input, we do not need to worry about losing key information for speech synthesis.
\end{comment}

==> 6_Acknowledgements.tex <==
\section*{ACKNOWLEDGMENT}
\label{sec:acknowledgements}
This work was supported by the project `Alchemist Brain to X (B2X) Project' through
the Ministry of Trade, Industry and Energy (MOTIE), South Korea, under Grant 20012355 and NTIS 1415181023. 
